RAWDet-7: A Multi-Scenario Benchmark for Object Detection and Description on Quantized RAW Images

Most vision models are trained on RGB images processed through ISP pipelines optimized for human perception, which can discard sensor-level information useful for machine reasoning. RAW images preserve unprocessed scene data, enabling models to leverage richer cues for both object detection and object description, capturing fine-grained details, spatial relationships, and contextual information often lost in processed images. To support research in this domain, we introduce RAWDet-7, a large-scale dataset of ~25k training and 7.6k test RAW images collected across diverse cameras, lighting conditions, and environments, densely annotated for seven object categories following MS-COCO and LVIS conventions. In addition, we provide object-level descriptions derived from the corresponding high-resolution sRGB images, facilitating the study of object-level information preservation under RAW image processing and low-bit quantization. The dataset allows evaluation under simulated 4-bit, 6-bit, and 8-bit quantization, reflecting realistic sensor constraints, and provides a benchmark for studying detection performance, description quality & detail, and generalization in low-bit RAW image processing. Dataset & code upon acceptance.

==> tex_files_for_tables/dataset_statistic.tex <==
% \begin{table*}
% \renewcommand{\arraystretch}{1.3}

% \centering
% \caption{Dataset Statistics}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c c c c c c c c c c c c}
% \toprule
% Dataset & Bit Depth&Car&	Bicycle&	Motorcycle&	Person&	Tram&	Bus&	Truck& Training Images & Testing Images\\
% %\hline\hline
% \midrule
% Pascal Raw & 12 &4007&3316&106&6054&21&14&113&2129 & 2130\\

% Raw NOD Nikon & 14 &3752&5044&1597&17768&24&188&132&3374 & 843\\

% Raw NOD Sony & 14 &3114&3964&1273&14412&15&85&111&3312 & 828\\

% RAOD & 24 &153380&6003&7398&39005&508&3665&8070&15973& 3869\\

% Zurich & 10 &968&153&43&496&5&14&59&107 & 26\\
% \bottomrule
% \end{tabular}}
% \hfill % maximize the horizontal separation
% \end{table*}

\begin{table}[h!]
\centering
\caption{Dataset Statistics: Breakdown of instances in the total vs individual datasets}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l c c c c c c c c c c@{}}
\toprule
Dataset & Bit Depth & Person & Bicycle & Motorcycle & Car & Bus & Truck & Tram & Training Images & Test Images\\
 \midrule
Pascal Raw &12& 5543 & 853 & 98 & 3555 & 12 & 101 & 10 & 2129 & 2130\\
Zurich  &10& 356 & 112 & 36 & 788 & 14 & 53 & 5 & 0 & 142\\
Raw-NOD-Nikon &14& 16274 & 4087 & 1419 & 3446 & 184 & 126 & 24 & 3374 & 843 \\
Raw-NOD-Sony &14& 13299 & 3327 & 1155 & 2916 & 82 & 110 & 14 & 3311 & 828\\
RAOD &24& 31555 & 4449 & 6706 & 138492 & 3619 & 7862 & 486 & 15968 & 3869 \\
\midrule
\textbf{Consolidated} &-& 67027 & 12828 & 9414 & 149197 & 3911& 8252&539 & 24888 & 7696 \\
\bottomrule
% maximize the horizontal separation
\end{tabular}}
\label{tab:8x5}
\end{table}

